Inductive Logic Programming via Differentiable Deep Neural Logic Networks

We propose a novel paradigm for solving Inductive Logic Programming (ILP) problems via deep recurrent neural networks. This proposed ILP solver is designed based on differentiable implementation of the deduction via forward chaining. In contrast to the majority of past methods, instead of searching through the space of possible first-order logic rules by using some restrictive rule templates, we directly learn the symbolic logical predicate rules by introducing a novel differentiable Neural Logic (dNL) network. The proposed dNL network is able to learn and represent Boolean functions efficiently and in an explicit manner. We show that the proposed dNL-ILP solver supports desirable features such as recursion and predicate invention. Further, we investigate the performance of the proposed ILP solver in classification tasks involving benchmark relational datasets. In particular, we show that our proposed method outperforms the state of the art ILP solvers in classification tasks for Mutagenesis, Cora and IMDB datasets.

==> Arithmetics.tex <==
Binary arithmetic tasks are among the widely used experiments in the topic of algorithm and pattern learning via DNNs. While binary operations are quite easy to learn for small size binary numbers, learning becomes very difficult as the size increases. This problem has been tackled in two different ways. In the feed-forward approach, the models are designed such that the complete input stream of symbols is processed sequentially through multiple layers and the output of the last layer generates the stream of symbols corresponding to the desired result of the arithmetic operation all at once (e.g.,\cite{kaiser2015neural}).
% 
Alternatively, this problem can be looked at as a case of the sequence-to-sequence learning problem (\cite{graves2014neural}) where we first process the input symbols one by one using a recurrent cell (e.g., an LSTM cell) and then another recurrent cell generates the output sequence of symbols sequentially while accessing all the outputs of the first recurrent layer generated at each time stamp. Various attention  mechanisms  and memory access models have also been proposed to improve the performance of these recurrent networks \cite{luong2015effective}.
%
To evaluate our proposed logical layers in such a standard task, we first consider the  addition of two long binary numbers. We represent each digit in a one-hot vector of depth=4 to denote $\{0,1,+,space\}$ symbols, where $space$ is used for padding the sequences to have identical lengths. 
%A typical input/output pair bis shown in below
%\begin{center}
%	\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|}
%		\hline 
%		input stream & 1 & 0& 1& 0 & 1 & + & 1   & 1 & &  &    \\
%		\hline
%		output stream & 1& 1& 0 & 0& 0&  & &  & &  &    \\
%		\hline
%	\end{tabular}
%\end{center} 
Among the existing models in the literature, Neural GPU model \cite{kaiser2015neural} proved to be the most successful approach in solving such problems using a feed-forward network.
% 
In \cite{kaiser2015neural}, the authors proposed a model consisted of a multi-layer feed-forward network where each layer is designed using a recurrent convolutional GRU cell \cite{cho2014properties}.This model (combined with curriculum learning) is reported to attain 100\% accuracy for the addition of up to 2000 long binary numbers. 
%
In our experiments, we were also able to achieve 100\% accuracy in binary addition of any lengths we tested (we did not test above 200 long sequences though). 
%
We trained the Neural GPU using its default set of parameters but for our model we used two layers of SXOR logic with length 100 each followed by a set of DNF-CNF layers each with a hidden layer of size 50 in our feed-forward model (as shown in Fig.~\ref{fig:arithmodelFF}). Table~\ref{tbl:binaryfeedforward} compares the speed of the convergence for the two models by displaying the number of the training samples required to reach a certain level of accuracy for $n=10$ and $n=20$ digits inputs. As Table \ref{tbl:binaryfeedforward} suggests while both models are capable of reaching 100\% accuracy, our proposed model converges much faster. Our experiments show that our model reaches 99\% accuracy for various lengths in less than 200k training samples. However, it usually requires much more training samples to reach the 100\% accuracy level.
%
\begin{table}[h]
	\caption{Size of required training samples to reach certain levels of accuracy}
	\label{tbl:binaryfeedforward}
	\centering 
	\begin{tabular} {|c||c| c|c|}
		\hline
		Model   & 75\% & 90\% & 100\%  \\		
		\hline
		Neural GPU (n=10) & 77k  & 400k & 490k    \\ \hline
		Logic CNF-DNF (n=10) & 4k  & 25k & 260k    \\ \hline
		Neural GPU (n=20) & 400k  & 448k & 830k    \\ \hline
		Logic CNF-DNF (n=20) & 8k  & 45k & 610k    \\ \hline
	\end{tabular}
\end{table}
% 
%A more challenging task, however,  is to learn this kinds of problems in a recurrent fashion such that the network produces the output stream one symbol at a time using the same recurrent cell. As we mentioned, most state of the art methods uses some fancy ways of attention modeling and memory access to learn these recurrent algorithmic tasks.  While all those approaches are also applicable in our logical learning system, we focus on a simple model of only one recurrent cell that accesses the input stream at any time stamp and generate one symbol of the output alphabet at each timestamp as depicted in figure \ref{fig:arithmodelRNN}. We use a simple vanilla logical recurrent (LVRNN) (Fig. \ref{fig:logicRNN}) as our recurrent cell and we test this model for the task of adding two long decimal numbers. \colorbox{red}{probably have to remove or reduce this part of experiment}
%
\begin{figure}[htb]
	\label{fig:arithmodel}
	\centering     %%% not \center
	\subfigure[Feed-Forward Model ]{\label{fig:arithmodelFF}\includegraphics[width=45mm]{Feedforwardmodel.pdf}}
	\hspace{1mm}
	\subfigure[Recurrent Model]{\label{fig:arithmodelRNN}\includegraphics[width=55mm]{rnnmodel.pdf}}
	\caption{Feed-Forward and recurrent models used in our experiments}
\end{figure}

==> LogicLayer.tex <==
Throughout this paper, we use 1 (True) and 0 (False) representations for the two states of a binary variable. The basic Boolean functions of two Boolean variables $x$ and $y$ can be written as
\begin{subequations}
\begin{align}\label{eq:BoolAlgebra}
\bar{x} &\quad=\quad  1 - x  \qquad,\qquad  \bar{y} =  1 - y \\
x \bigwedge y &\quad=\quad   xy \\
x \bigvee y &\quad=\quad \overline{\bar{x} \bigwedge \bar{y}}   \quad=\quad 1 - ( 1 - x )( 1 - y)  
\end{align}
\end{subequations}
%where $\otimes$ denotes the exclusive OR operation. 
%
This algebraic representation of the Boolean logic allows us to manipulate the logical expressions similar to the regular arithmetic. 
%
Let $\bx \in \{0,1\}^n$ be the input vector in a typical logical layer, and the Boolean vector $\by \in \{0,1\}^m$ be the corresponding layer output. 
%
For the conjunctive layer, our goal is to learn $m$ conjunction functions over $ \{0,1\}^n$ such that each function uses an arbitrary subset of the binary variables in $\bx$, e.g., $y_0 = x_1 \bigwedge x_7 \bigwedge x_8$ and $y_1 = x_0 \bigwedge x_1 \bigwedge x_2 \bigwedge x_7$ and so on. 
%
To learn such representations, we introduce membership weights $w_i^{(j)}$ to the network where $j \in \{1,\dots,m\}$ and $i \in \{1,\dots,n\}$. We define the layer outputs as
\begin{equation}\label{eq:conj}
y_{conj}^{(j)} = \prod_{i=1}^{n} \big( 1 - \sigma ( w_i^{(j)} )(1 - x_i )\big).
\end{equation}
%
where $\sigma(.)$ is a squashing function which limited the membership weights to the range of $[0,1]$. We consider two types of the squashing functions; hard thresholding via two times application of the relu functions , i.e. $\sigma(w) = \text{relu}( 1 - \text{relu} (1 - w))$ or alternatively soft thresholding sigmoid function in the form of $\sigma(w) = sigmoid( c * w)$ where we choose constant $c > 1$ to encourage the membership weights to move faster towards either $0$ (no membership) or $1$ (full membership).
%
While both methods works, we realized the sigmoid scaling method is more stable and allows us to use higher learning rates.
%
It is easy to see how the membership weight principle in (\ref{eq:conj}) works. Whenever $w_i^{(j)}$ converges to zero, the $i^{th}$ term in the product goes to 1 and hence the effect of $x_i$ in the expression vanishes. On the other hand, the corresponding term is reduced to $x_i$ if the membership weight goes to 1. 
%
In the actual implementation\footnote{Tensorflow implementations of the algorithms in the paper is available at \url{https://github.com/xxx/xxx}}, for the speed and stability, we replaced the product with the summation of the logarithm terms, i.e. $y_{CONJ}^{(j)} = \text{exp} (\sum ^{n}  \log( \epsilon +  1 -\sigma(  w_i^{(j)}) (1 - x_i )\big))$, where $\epsilon$ is a small constant added for stability. 
%Further, when the dimension of the input vector is large, we may notice that even for values of $\sigma(w)$ close to $1$, the product term would be very close to zero which makes the learning slow. In order to fix this, we can reduce the effect of the input vector dimension by dividing the 
%
This operation is always valid since all the weights and inputs are in the range $[0,1]$. 
%
The resulting layer has the same complexity of a single layer perceptron in terms of the number of multiplication/addition. However, note that our logic layer incurs a subtle extra cost due to the application of logarithm and exponential functions to convert the multiplication to addition.
%

The disjunctive layer can be defined similarly using the membership weights. We define the disjunctive layer using the De Morgan Law as
\begin{align}\label{eq:disj}
y_{DISJ}^{(j)} = 1 - \prod_{i=1}^{n}  ( 1 - \sigma( w_i^{(j)} ) \,x_i  ).
\end{align}
%
In design of new layers, we leverage the property that any arbitrary complex Boolean function can be expressed in standard Disjunctive Normal Form (DNF) or in Conjunctive Normal Form (CNF). 
%
In DNF form, the Boolean function is expressed by the disjunction of the sub-expressions which are consisted of only conjunctions. 
%
This is correspond to applying our proposed disjunction layer on the output of a conjunction layer.
To represent a Boolean function, we cascade our proposed disjunction and conjunction layers in (\ref{eq:disj}) and (\ref{eq:conj}) to form a DNF layer ( $ \text{DNF}(\bx) = \text{DISJ}( \text{CONJ} (\bx) )$ ) or in reverse to form a CNF layer ($\text{CNF}(\bx) = \text{CONJ}( \text{DISJ} (\bx) )$)

%We combine our proposed conjunctive and disjunctive layers to form two new multilayer structures denoted as CNF and DNF layers. then combine these two multi-layers to form a new CNF-DNF layer. This new layer would result in low complexity networks in learning complex expressions. 
%
%While 
The total number of logical functions over a Boolean input vector $\bx \in \{0,1\}^n$ is very large (i.e. $2^{2^n}$). Further, %\color{red}it is known that many of those functions can be expressed via a small number of clauses using CNF or DNF forms\color{black}. However, 
 in some cases, a simple clause in one of those standard forms can lead to an exponential number of clauses when expressed in the other form~\footnote{We can always convert CNF to DNF form and vice versa using De Morgan's Law.}. For example, it is easy to verify that converting  $(x_1 \bigvee x_2 ) \bigwedge (x_3 \bigvee x_4)\bigwedge\dots\bigwedge(x_{n-1} \bigvee x_{n} )$ to DNF leads to $2^{\frac{n}{2}}$ number of clauses. As such, it seems intuitive to increase the learning capability of the model by combining the CNF and DNF layers using the disjunction operator to create a CNF+DNF layer as
\begin{align}\label{eq:DNF-CNF}
y_{\text{DNF+CNF}}(\bx) \,&=\, \text{CNF}(\bx) \bigvee \text{DNF}(\bx) \\&=\, 1 - \big(1-\text{CNF}(\bx)\big) \big( 1-\text{DNF}(\bx)\big)
\end{align}
The combined CNF+DNF layer gives the model the freedom to use each of the standard forms that is more suitable to represent a Boolean function.

==> formulation.tex <==
In the most basic form, ICA assume the multivariate observation data is generated by a linear combination of the independent components we call source, i.e. $\bx^{(i)} = \bA \bs^{(i)}$. While this problem has been studied extensively [ref] and has been solved with theoretical guaranties, for the more general form of the problem in presence of noise and especially where the sources are mixed using non-linear functions instead of linear form, there has not been much success. 
